A Deep Learning Framework for Lifelong Machine Learning

Humans can learn a variety of concepts and skills incrementally over the course of their lives while exhibiting many desirable properties, such as continual learning without forgetting, forward transfer and backward transfer of knowledge, and learning a new concept or task with only a few examples. Several lines of machine learning research, such as lifelong machine learning, few-shot learning, and transfer learning attempt to capture these properties. However, most previous approaches can only demonstrate subsets of these properties, often by different complex mechanisms. In this work, we propose a simple yet powerful unified deep learning framework that supports almost all of these properties and approaches through one central mechanism. Experiments on toy examples support our claims. We also draw connections between many peculiarities of human learning (such as memory loss and "rain man") and our framework. As academics, we often lack resources required to build and train, deep neural networks with billions of parameters on hundreds of TPUs. Thus, while our framework is still conceptual, and our experiment results are surely not SOTA, we hope that this unified lifelong learning framework inspires new work towards large-scale experiments and understanding human learning in general. This paper is summarized in two short YouTube videos: https://youtu.be/gCuUyGETbTU (part 1) and https://youtu.be/XsaGI01b-1o (part 2).

==> old/sec_4_connections.tex <==
\section{Close Connections to Other Learning Settings}
\label{sec:connections}

In this section we will describe how our unified framework can be applied to learning settings beyond LLL and fully connected neural networks. Several of these learning settings are closely related to LLL in their setup and scope: multi-task learning, curriculum learning, few-shot learning, and transfer learning. We will provide a brief discussion of their connections to our framework. Other learning settings are based on the type of model being used: convolutional networks, deep random networks, and capsule networks. For each of these will will discuss how our framework could be applied to them or is otherwise connected to them.

% Multi-Task and Curriculum Learning
%   sec:rd_curriculum
% Few-shot Learning and Bongard Problems
%   sec:rd_bongard
% Pre-Training
%   sec:pretraining
% Transfer Learning
%   sec:transferlearning
% Meta-Learning
%   sec:metalearning
% Extension to Convolutional Networks
%   sec:rd_cnns
% Deep Random Networks
%   sec:rd_rand
% Capsule Networks
%   sec:rd_capsules

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-Task and Curriculum Learning}
\label{sec:rd_curriculum}

Special cases of LLL are multi-task learning \citep{caruana1997multitask} and curriculum learning \citep{bengio2009curriculum}. In multi-task learning, all $(T_{i}, D_{i})$ are provided together, allowing the model to be trained on all tasks at the same time. In curriculum learning, all data is similarly made available, but the problem is to identify the optimal order in which to train on data for the most efficient and effective learning. 
An example of an intuitive type of curriculum is to learn tasks from ``easy'' to ``hard'' \citep{elman1993learning}, similar to the way humans often learn new concepts. This idea is reflected in Algorithm \ref{alg:curriculum_learning}.

\begin{algorithm}[H]
    \SetAlgoLined
    \tcp{Assume a pool of tasks to learn from}
    \While{pool is not empty}{
        Select the best task, $T_{best}$ \tcp{the easiest, for example}
        \textcolor{Cerulean}{$\CIRCLE$} Apply Alg.~\ref{alg:new_task} to learn $T_{best}$\;
        \textcolor{Cerulean}{$\CIRCLE$} Apply Alg.~\ref{alg:confusion_reduction} \tcp{reduce confusion if necessary}
        Remove $T_{best}$ from pool\;
    }
    \textcolor{Cerulean}{$\CIRCLE$} Apply Alg.~\ref{alg:overall_refinement} \tcp{final refinement of all tasks}
\caption{Curriculum Learning}
\label{alg:curriculum_learning}
\end{algorithm}

While research has been done on combining active and curriculum learning with LLL \citep{ruvolo2013active, sun2018active, de2019continual}, we suspect more is needed.
Research directions to further develop these ideas include:
\begin{enumerate}
    \item Understanding how a task selection mechanisms might work with a weight consolidation policy, where transference between tasks can be more explicitly controlled.
    \item Developing or learning to identify a taxonomy over samples to better construct curricula such as simple to complex.
    \item Given that the general task type to be learned is known, can we automatically construct primitive pre-training samples. For example, if we are training a LLL more for hand-written characters, pre-training on simple strokes may help. 
    \item How much can an optimized curriculum reduce data requirements and improve few-shot learning performance?
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Few-shot Learning and Bongard Problems}
\label{sec:rd_bongard}

%
\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.75\textwidth]{figs/BP_examples.pdf}
    \caption{Two examples of Bongard problems. (a) BP \#5 is simple, where the rule is polygonal shapes on the left and curvilinear shapes on the right. (b) BP \#99 is quite hard, where the rule is that larger shapes formed by connecting similar small shapes overlap vs. the larger shapes do not overlap. Such highly abstract rules are common among BPs. For such difficult BPs (including that in Figure~\ref{fig:bp57}), we find that for both humans and machine learning, adding more training samples often does not help, and rather it takes a ``stroke of insight'' or sufficiently similar previously acquired knowledge to solve it. We can easily generate more test data using the desired rule to test any learning algorithms after trained on a small number of data.}
    \label{fig:BP_examples}
\end{figure}

LLL and curriculum learning have great potential to achieve few-shot learning of difficult concepts, which humans are often capable of doing. By learning relevant easier concepts earlier with LLL, later harder ones could be learned with many fewer examples via forward transfer of knowledge. 

Humans can often discover the underlying rules and patterns of complex concepts with only a few examples.  
We can use Bongard Problems (BPs) \citep{bongard1967problem}
to illustrate this\footnote{A collection of BPs can be found here: http://www.foundalis.com/res/bps/bpidx.htm.}.
A particular BP asks a human to recognize the underlying rule of classification with
only 6 examples on the left (say they are positive) and 6 examples on the right (negative samples).   
Two such BPs are shown in Figure~\ref{fig:BP_examples},
where (a) is a simple BP and (b) is a difficult BP for humans.
To solve BPs, humans often require identifying highly abstract rules learned earlier in their lives (or in easier BPs). 
Some form of LLL of many visual abstract concepts and shapes must likely have happened in humans so that they can accomplish BPs well with only 12 examples in total.  

We can outline a possible few-shot learning process to learn such BPs in our LLL framework, in a curriculum-like fashion. 
First, we can train (or pre-train) on simpler tasks to recognize simpler shapes.
Next, harder and more complex visual shapes and BPs would be 
trained. 
This idea of using curriculum learning to ``working up to'' more difficult BPs is reflected in Figure~\ref{fig:Curriculum_BP}. 
In this illustrative example, we feed previous class labels (the output nodes) into nodes of new tasks to provide opportunity for forward transfer of knowledge. With this approach, BPs could be solved with fewer examples, as shown by \citet{yun2020deeper}. 
Note that in this illustrative example, the networks of subsequent tasks can have different and increasing depths in order to solve more difficult problems after easier problems are learned.  

%It is also important to note that while the original goal of solving BPs is to discover rules (expressed in natural language) for classification, here we can simply test our learning model by using predictive accuracy on additional test samples following the intended rule.
To solve difficult BPs with a few examples (such as BP \#99 in Figure~\ref{fig:BP_examples}b), the importance of forward transfer of knowledge is crucial. If a person cannot solve BP \#99 (or other hard BPs) in several minutes, normally more training data would not help much.  Often ``a flash of inspiration'' or ``Aha!'' moment would suddenly occur and the problem is solved.  This is because a person has learned probably thousands or tens of thousands of concepts and abstract relations in his/her life, and the correct knowledge is suddenly combined to solve the hard BP.   

\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.85\textwidth]{figs/BP_curric_learning.pdf}
    \caption{An illustrative example of curriculum learning to work up to solving Bongard problems with a small number of positive and negative examples. After learning to differentiate between basic strokes types, shapes, and possibly other early tasks, these representations including the output and hidden layers can be transferred to $T_{k}$ to possibly solving BPs such as BP\#5 (sharp angles vs. smooth curves) with a few examples. 
    This process can continue to allow us to solve a more complex visual reasoning problem with a few samples. Note that networks of subsequent tasks can have increasing depths in order to solve harder BPs after easier ones have been learned.}
    \label{fig:Curriculum_BP}
\end{figure} 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Pre-Training Methods}
\label{sec:pretraining}

Pre-training is a ubiquitous process in deep learning \citep{devlinetal2019bert, girshick2014rich, wang2015unsupervised}. 
In computer vision (CV), nearly all state-of-the-art approaches rely on pre-training on a non-target task for which there is abundant data \citep{mahajan2018exploring}, such as the ImageNet dataset \citep{russakovsky2015imagenet}. Pre-trained CV models such as VGG-16 \citep{simonyan2014very} have been shared to the public allowing anyone to fine-tune their model to achieve otherwise infeasible performance on their target task. Due to the reduced need for target task training data, using pre-trained CV models is also a common approach to few-shot learning. \citep{ramalho2019empirical}.
In natural language processing, pre-trained language models have recently become popular \citep{conneau2017supervised, peters2018deep, devlinetal2019bert}. For example, BERT (Bidirectional Encoder Representations from Transformers) \citep{devlinetal2019bert}, has shown that state-of-the-art performance can be attained on several different NLP tasks with a single pre-trained model.


With pre-training, often a large neural network is first trained on one or more tasks with very large labeled training datasets.
The trained neural network would be then frozen, 
and a smaller network stacked on top of the large network and trained 
for improved performance on target tasks. From the perspective of our framework, the consolidation values of the smaller networks would be considered unfrozen for training.   

Pre-training can thus be viewed as certain weight consolidation policies in our LLL framework. 
The main difference is that most of our weight consolidation algorithms in the last section apply to weights per tasks, or column-wise in our figures, while for pre-training, consolidation is layer-wise. An interesting research topic would thus be to consider designing consolidation policies which perform both layer-wise and column-wise consolidation based on the task at hand.

A natural way to fine-tune the consolidation policy when tuning on the target task is to consider how much to unfreeze each layer. Instead of simply tuning the output layer or tuning the entire network, we can interpolate between these two policies, to allow 
gradual unfreezing of layers in the network to best adapt to the target task 
without losing the generalization benefits of pre-training.  See \citep{erhan2010does} for an example of such directions. 

Deep random networks are a another example of layer-wise consolidation policies.  See Section~\ref{sec:rd_rand} for more details. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Transfer Learning and Meta-Learning}
\label{sec:transferlearning}

Transfer learning is closely related to LLL as well as curriculum learning, few-shot learning, and pre-training. It is explicitly concerned with aiding the learning of a task by exploiting previously-acquired knowledge \citep{de2019continual}. With respect to LLL, it is solely concerned with forward transfer and not maintaining or improving previous task performance.

Aspects of our framework with application to pure transfer learning thus include continual learning (Section~\ref{sec:expansion}) and forward transfer (Section~\ref{sec:forwardtransfer}). After learning an initial set of tasks, being able to learn the new task may require expanding the network depending on the difficulty. The techniques discussed for forward transfer can be used to initialize these newly added weights as well as apply the appropriate consolidation to avoid negative transfer and maximize positive transfer.

Meta-learning is another learning setting similar to transfer learning. Instead of directly using previous task knowledge to help learn a known new task, we instead use the previous tasks to learn \textit{how} to learn on an unknown new task \citep{hospedales2020meta}. By optimizing the learning process, we can learn new tasks faster, with higher performance, and with less data. This kind of learning can occur in many ways, including:
\begin{enumerate}
    \item Learning a good parameter initialization. In Section~\ref{sec:forwardtransfer} we discuss methods for initializing new task weights to speed up learning.
    
    \item Identifying a good architecture. In Section~\ref{sec:expansion} we consider estimating the additional network size required to learn a new task to a sufficient performance level. This estimate can be based on both how difficult the task is as well as how similar it is to previous tasks.
    
    \item Learning to compute task similarity. If we perform meta-learning in preparation of learning \textit{many} tasks (as in LLL, multi-task learning, or continual learning), we can consider meta-learning the task similarity metric, $sim$ (Section~\ref{sec:forwardtransfer}). This would have many downstream benefits, including improve parameter initialization, better estimates of required network expansion, and better informed consolidation policies.
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Convolutional Networks}
\label{sec:rd_cnns}

% mammals and birds

While we have so far considered our framework as applied to fully connected feed-forward networks, we can also consider its application to convolutional neural networks (CNNs). Training on image tasks is often performed with resource-intensive batch learning, while our framework would allow for increased efficiency while being careful to maintain the high performance associated with batch learning. For example, our framework could first learn to classify mammals as $T_{1}$, and birds as $T_{2}$ (as shown in Figure~\ref{fig:batchvslll}). This is closer to human learning, as we never learn to recognize all objects in a single sitting, which is how training commonly occurs on the popular ImageNet dataset \citep{Imagenet} for example. Instead, we are exposed to different things over the course of our lives. This would be done without re-using data for $T_{1}$ or forgetting $T_{1}$, while allowing forward transfer from $T_{1}$ to $T_{2}$ (ways of achieving these properties, among others, are discussed in Section~\ref{sec:framework}).

\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.8\textwidth]{figs/Batch_vs_lll.pdf}
    \caption{A comparison between batch learning generally commonly applied for computer vision, and the more human-like LLL approach. With batch learning, all data is combined and trained together in one sitting. With LLL, improved memory and computational efficiency can be attained by training on individual tasks (such as mammals in $T_{1}$ and then birds in $T_{2}$) in succession. This is done without requiring previous task data or forgetting of previous tasks, similar to humans.}
    \label{fig:batchvslll}
\end{figure}

Adapting the consolidation mechanism to work with CNNs can be done as follows. In the fully connected networks, each consolidation value $\pmb{b}_{i}$ corresponds to a weight in a densely connected layer, but in CNNs, each $\pmb{b}_{i}$ corresponds to a filter. A filter is essentially a set of weights which takes the representation from the previous layer (feature maps), and transforms it into a new feature map. Large $\pmb{b}$ on a filter means the filter cannot be easily modified during learning. With the consolidation mechanism described for CNNs, we can now consider how to achieve the various LLL properties in CNNs:

\textbf{Continual learning of new tasks}. To extend the network for new tasks, we now add columns of convolutional filters, as reflected in Figure~\ref{fig:cnn}b (solid links). Transfer links between tasks (dashed links in Figure~\ref{fig:cnn}b) now correspond to filters. The resultant feature maps of these ``transfer filters'' are concatenated with the feature maps in the new task column.  For more difficult tasks, we can add a greater number of filters (instead of a greater number of nodes). Instead of pruning weights or nodes, we can now prune filters.

\textbf{Non-forgetting}. Controlling non-forgetting means that large values in $\pmb{b}$ are applied to filters of previous tasks so they are not easily modifiable. See dotted links of Figure~\ref{fig:cnn}.

\textbf{Forward transfer}. The two methods of encouraging forward transfer also work with CNNs. First, instead of ``copying'' weights for previous tasks when similar to the new task, we can now copy over filter values. This can be done using similar ideas to those laid out in Section~\ref{sec:forwardtransfer}. Second, we can encourage forward transfer and avoid negative transfer through controlling flexibility of the transfer filters (dashed links in Figure~\ref{fig:cnn}b). When these filters are initialized to zero and the $\pmb{b}$ values are very large, the new task can be prevented from using knowledge from the previous task.



\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.8\textwidth]{figs/cnn_version.pdf}
    \caption{A simplified visualization of how our framework can be applied to convolutional networks. In (a) is a diagram of our consolidation mechanism and expansion being applied for learning two tasks with a fully connected network. In (b) is the corresponding CNN with the same high-level topology as (a) being applied to e.g. mammals for $T_{1}$ and birds for $T_{2}$. Links with unfilled arrow heads indicate filter weights, and links with filled arrow heads indicate weights between fully connected layers. Dotted (red) indicates large $\pmb{b}$ values, solid (blue) indicates $\pmb{b}$ values of 0, and dashed (green) indicates transfer links whose consolidation may depend on task similarity.}
    \label{fig:cnn}
\end{figure}

While dynamic CNN architectures for lifelong learning have been considered before, starting from the AlexNet architecture \citep{yoon2018lifelong, Imagenet}, we can consider taking a step further and considering more complex units like DenseNet blocks \citep{huang2017densely} or Inception modules \citep{szegedy2015going}. It is clear that almost all of the techniques discussed in this paper can be extended to CNNs and more complex networks allowing the desired LLL skills (such as non-forgetting, forward transfer, few-shot learning, and so on) to be obtained. However, much more future research on this would be needed. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Deep Random Networks}
\label{sec:rd_rand}


Another active research area that can be viewed from our LLL framework is deep random neural networks, which have been found to provide efficient learning with good generalization bounds \citep{rudi2017generalization, rosenfeld2019intriguing, gallicchio2020deep}. Their success derives from the surprising usefulness of random projections at tasks such as locality-sensitive hashing \citep{giryes2016deep, andoni2008near}.


The design of this lifelong learning approach, summarized in Algorithm~\ref{alg:rand_nn} is as follows: randomly initialize a neural network and permanently freeze all but the output layer (via the consolidation policy). To learn new tasks, only train the weights to the new output nodes. 

\begin{algorithm}[H]
    \SetAlgoLined
    Initialize a single random network \tcp{Gaussian weights have been proven to work well for this kind of approach \citep{giryes2016deep}}
    \textcolor{Cerulean}{$\CIRCLE$} Freeze all weights except for the output layer \tcp{dotted (red) weights in Figure~\ref{fig:rand_nn}}
    \textcolor{Cerulean}{$\CIRCLE$} Use Algorithms \ref{alg:forward_transfer}, \ref{alg:confusion_reduction}, \ref{alg:overall_refinement} during lifelong training on task sequence \tcp{for forward transfer, confusion reduction, and overall refinement respectively}
\caption{Learning using a Random Network}
\label{alg:rand_nn}
\end{algorithm}

This approach provides guaranteed non-forgetting. Other benefits include computational efficiency (only a minority of weights need to be tuned), and sample storage size efficiency (instead of storing whole samples, we can simply store the activation vectors at last hidden layer and skip a majority of inference during rehearsal).

With regard to this kind of approach, some possible research directions include:

\begin{enumerate}
    \item Unfreezing even just a small fraction of the weights was found to improve performance considerably \citep{rosenfeld2019intriguing}. If this is done, can we still maintain LLL skills that come with this approach such as guaranteed (or at least tightly bounded) non-forgetting and computational and storage efficiency?
    \item We can consider slowly unfreezing starting from the last hidden layer and moving towards the input as we learn more tasks, such as in Figure~\ref{fig:rand_nn} (a), (b), (c). Combined with overall refinement to prevent any forgetting of earlier tasks, this would allow the network to accommodate more difficult tasks while still maintaining some of the efficiency of a fully-frozen network.
    \item It would be an interesting research question to determine the optimal consolidation policy or schedule with which to progressively unfreeze layers. Should flexibility only be increased when we are unable to achieve sufficient performance on tasks?
    \item While weights can be frozen layer-wise, among unfrozen layers, we can still apply our LLL algorithms discussed earlier to freeze and unfreeze weights for new task learning without forgetting, forward- and backward-transfer, confusion reduction, and so on. That is, weights can be frozen and unfrozen layer-wise as well as task-wise according to the need. Figure~\ref{fig:rand_nn}d for example illustrates how confusion reduction might be performed when the original randomly initialized network is insufficient to resolve confusion. After resolving confusion, the newly added weights can be frozen similar to the others in their layers.
\end{enumerate}


\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.7\textwidth]{figs/rand_nn.pdf}
    \caption{Visualization of the deep random projection lifelong learning approach with possible iterative unfreezing shown in (a) to (b) to (c). Initially, all weights except for the output layer are frozen. Slowly, layers (starting from the near the output) are unfrozen (transitioning from dotted/red to solid/blue). In (d) is an example of how expansion with column-wise freezing and unfreezing can be used in the case where confusion (e.g. between $T_{1}$ and $T_{3}$) cannot be reduced with the original architecture. }
    \label{fig:rand_nn}
\end{figure}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Capsule Networks}
\label{sec:rd_capsules}

We believe that there is considerable overlap between capsule networks \citep{sabour2017dynamic, hinton2018matrix} and our LLL framework.  
Capsule networks emphasize modularity in neural network learning for computer vision; that is, capsules are a group of neurons that can accomplish certain CV tasks. In LLL, capsules are analogous to sub-networks (such as sub-networks for tasks 1, 2, 3 in Figure~\ref{fig:framework_p1}) for different tasks. Dynamic routing in capsule networks is analogous to forward- and backward-transfer links that connect different sub-networks in LLL. The main difference, in our view, is that LLL emphasizes that tasks are often learned in sequence, usually from simple to complex, over time.  For humans, LLL happens over many years.  Usually easier shapes would be learned earlier in life directly with supervised data, and then modules would be frozen to prevent forgetting (Section~\ref{sec:nonforgetting}), and its outputs can be used to learn more complex shapes. 
Of course human learning is not always done from simple to complex.  Often data from an earlier task can arrive later and an already-learned learned module must be updated. This is discussed in Sec~\ref{sec:conceptdrift}, where the weights for all other tasks are frozen to prevent forgetting while knowledge for a task is being updated with new data.


Figure~\ref{fig:capsule_like} illustrates the LLL of various vision tasks in a modular fashion. 
Note that here the ``modules'' can be neural networks, or other learning algorithms, as long as there is a consolidation parameter controlling how flexibly the module can be modified in learning.
The whole LLL process is complex, and various steps have been discussed in Section~\ref{sec:framework} and the previous parts of this section. 

\begin{figure}[ht]
    \centering
    % link to editable figure:
    \includegraphics[width=0.75\textwidth]{figs/caps_version.pdf}
    \caption{An illustrative example of learning multiple tasks of various complexity in LLL.  Often simpler tasks (such as lines) are learned earlier with training data (of lines).  The weights in their sub-networks or modules would be frozen to prevent forgetting, and their outputs would be forward-transferred (dashed links) to other modules to participate in learning other tasks (such as squares, roof, and house).  The weights between modules are also learned as in forward and backward transfer (Section~\ref{sec:forwardtransfer} and \ref{sec:backwardtransfer}), regularized by the consolidation values.  Sub-networks or modules are like capsules and links are like dynamic routing in capsule networks. Ideally LLL happens from simple to complex, but often can be episodic (Section~\ref{sec:conceptdrift}).  
    In the figure, solid links can be frozen or unfrozen based on the need. We also use the size of the module to roughly represent the complexity of the module, or the depths and number of nodes in the network capsules.  Note that here the ``modules'' can be neural networks, or other learning modules, as long as there is a consolidation parameter controlling how flexibly the module can be modified in learning.}
    \label{fig:capsule_like}
\end{figure}


A real-life example of how metaphoric ``capsules'' in human learning can be illustrated as follows: 
The design of houses is different between cultures, climates, and geographic locations, and evolves over time. 
Seeing a straw roof for the first time may be surprising to many people. After seeing a straw roof, the module for ``roof'' may be re-learned (while not forgetting other learned concepts, such as walls) after checking with local residents that straw can in fact be used for a roof (supervised example).  
This new knowledge improves the robustness of recognizing houses, whether they have shingles or straw roofs, and can provide forward transfer when learning to recognize further types of houses and roofs.

==> old/sec_5_parallels.tex <==
\section{Speculations on Parallels with Human Learning}
\label{sec:parallels}

As our framework focuses on controlling the flexibility of individual network weights, it is natural to ask how our approach lines up with the mammalian brain whose lifelong concept learning behaviours we are attempting to capture.
In this section we first consider how human brains may have come to exhibit the kind of procedures discussed in Section~\ref{sec:framework}. Next, we explore parallels between our framework and human learning with respect to several behavioural patterns listed in Table~\ref{tab:human}. For each of these, we will discuss how a similar behaviour can be exhibited by our framework with specific network sizes and consolidation policies, 
and how they may translate to what happens in the human brain at a similar level of abstraction. 

%%%%%%%%%%%%

\subsection{Reflecting on Nature vs. Nurture}

One may wonder how humans acquire such consolidation strategies as used in our LLL framework. This question is related to the long-standing debate on the influences of nature vs. nurture on human intelligence \citep{leahy1935nature, gazzaniga1992nature, kan2013nature}. Here we only reflect on the issue as it relates to our framework.  

We believe that some of the consolidation policies in Section~\ref{sec:framework} are a result of nature---intrinsic to the physiology of the brain and a product of natural evolution. This would include those relating to network expansion and pruning (Section\ref{sec:expansion}), non-forgetting (Section\ref{sec:nonforgetting}), forward transfer (Section\ref{sec:forwardtransfer}), adapting to concept drift (Section\ref{sec:conceptdrift}), and graceful forgetting (Section\ref{sec:gracefulforgetting}). Some effects of nature on learning take place in the following ways: People are born with many more free neurons and synapses than required in adulthood \citep{ackerman1992discovering} and appear to have an innate capacity for learning many concepts (and other skills for the world around them) without catastrophic forgetting
(perhaps using algorithms similar to those described in Section~\ref{sec:framework} and \ref{sec:connections}). 
As we develop, neurons will be pruned without our conscious effort, especially starting around adolescence \citep{sisk2005pubertal}. Throughout adulthood, graceful forgetting, refinement of existing concepts, and adapting to slowly shifting concepts and environments naturally occurs \citep{ackerman1992discovering, mcewen2010stress}.


In contrast, learning specific concepts and knowledge from data are more likely to be the result of nurture---they are things we must learn (such as recognizing different animals, shapes, and fruits). However, a person can perhaps consciously modify their nature-provided algorithms by performing meta-learning and changing consolidation policies. An example of this is memory training and explicit rehearsal.  This is  analogous to re-training of a specific concept with additional data while slowly increasing the $\pmb{b}$ values for the concept in our framework.


%%%%%%%%%%%%
\subsection{Interpreting Human Learning Properties}

We observe that our LLL framework seems to be able to explain human LLL well, with many properties discussed below and summarized in Table~\ref{tab:human}. 
Here we broaden our scope to general human learning of tasks and skills, instead of restricted to supervised learning. 
Further research is of course needed to determine to what extent human brains actually use mechanisms similar to those discussed in this paper.

\textbf{Resourceful and versatile}. Ideally, human learning allows us to acquire a lot of knowledge, yet be flexible enough to adapt to new experiences and make meaningful connections between experiences.
This is analogous to our framework in which the network has unlimited free units for new tasks (Section~\ref{sec:expansion}), can use previous knowledge to learn new tasks (Section~\ref{sec:forwardtransfer}), will not likely forget previous tasks while learning new ones (Section~\ref{sec:nonforgetting}), and can use new knowledge to refine old skills (Section~\ref{sec:backwardtransfer}).

\textbf{Memory loss}.
In Section~\ref{sec:nonforgetting}, we describe how by setting values in $\pmb{b}$ for previous tasks to be large (freezing), previous tasks will not be easily forgotten. However, if not, ``memory loss'' can gradually happen.  This can also happen when the available free units are limited, so that graceful forgetting (Section~\ref{sec:gracefulforgetting}) must happen in order to learn new tasks. If the kind of pruning performed for graceful forgetting is too aggressive, further detrimental memory loss may occur.

\textbf{Sleep deprived}. The human brain is suspected of performing important memory-related processes during sleep, and sleep deprivation has been observed to be detrimental to cognitive performance related to memory \citep{walker2010sleep, killgore2010effects}. Confusion reduction and backward transfer are important stages of our proposed approach which use rehearsal (functionally similar to memory replay), where the model is exposed to samples from past tasks in order to perform fine-tuning to achieve various properties (Section~\ref{sec:confusionreduction} and \ref{sec:backwardtransfer}). Without these rehearsal-employing steps, the model may be less able to distinguish between samples of similar classes. Additionally, the ability to identify connections between newer tasks and older ones will be lost, so that potentially useful newly acquired skills cannot benefit older tasks. In addition, when the brain is ``tired'' and not well-rested, this may be analogous to poor optimization of policies in our framework (and in all machine learning algorithms). If optimization is not thorough in Equation~\ref{eqn:loss}, performance would be poor in all aspects of LLL. 


\textbf{``Rain man''}.
If values in $\pmb{b}$ for previous tasks (Section~\ref{sec:nonforgetting}) are set to very large to achieve non-forgetting, and no connections are made between previous and new tasks, the knowledge transfer (Section~\ref{sec:forwardtransfer} and \ref{sec:backwardtransfer}) will likely not happen.  
This is reminiscent of Kim Peek, who was able to remember vast amounts of information, but performed poorly at abstraction-related tasks that require connecting unrelated skills and information and was the inspiration for the main character of the movie \textit{Rain Man} \citep{treffert2005inside}.


\textbf{Alzheimer's disease}. Alzheimer's disease is a highly complex neurological disease and is not fully understood by the medical community. However, an early stage of Alzheimer's disease is usually characterized by good memory on events years ago but poor on recent events \citep{tierney1996prediction}. This can be modeled in our framework by a small number of new neurons for new tasks and a very large $\pmb{b}$ values for old ones. 


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}llll@{}}
    \toprule
    \textbf{Behaviour} & \textbf{\# of neurons} & \textbf{$\pmb{b}$-setting policy} \\ \midrule
    \textbf{Resourceful and versatile} & large & large $\pmb{b}$ for non-forgetting (Sec.~\ref{sec:nonforgetting}), small $\pmb{b}$ for transfer (Sec.~\ref{sec:forwardtransfer}, \ref{sec:backwardtransfer}) \\
    \textbf{Memory loss} & small & small $\pmb{b}$ for previous tasks (Sec.~\ref{sec:nonforgetting}) and aggressive pruning  (Sec.~\ref{sec:gracefulforgetting})\\
    \textbf{Sleep deprived} & - & poor optimization of Eq.~\ref{eqn:loss} and application of consolidation polities\\
    \textbf{``Rain man''} & large & large $\pmb{b}$ for old tasks (Sec.~\ref{sec:nonforgetting}) and transfer links (Sec.~\ref{sec:forwardtransfer}, \ref{sec:backwardtransfer}) \\
    \textbf{Alzheimer’s disease} & small/shrinking & large $\pmb{b}$ for oldest memories (Sec.~\ref{sec:nonforgetting}) and aggressive pruning  (Sec.~\ref{sec:gracefulforgetting}) \\ \bottomrule
    \end{tabular}%
    }
    \caption{Correspondences between settings in our LLL framework and human behavioural descriptions. For example, being able to transfer knowledge across concepts and from old concepts to a newly encountered one allows us to be versatile.
    Here we broaden our scope to general human learning of tasks and skills, not restricting to supervised learning. }
    \label{tab:human}
\end{table}

==> tables/skills.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{llllll}
        \hline
        \textbf{Property} & \textbf{Replay-based} & \textbf{Regularization-based} & \textbf{Dynamic architecture-based} & \textbf{Our framework} & \textbf{Human learning} \\ \hline
        \textbf{Continual learning and testing} & good & good & good & good & good \\
        \textbf{Non-forgetting} & good & poor/okay & good & good & good \\
        \textbf{Forward transfer} & okay/good & okay/good & good & good & good \\
        \textbf{Few-shot learning} & poor & poor/okay & poor & good & good \\
        \textbf{Backward transfer} & good & poor & poor/okay & good* & good  \\
        \textbf{Adapting to concept update/drift} & good & poor & poor/okay & good* & good  \\
        \textbf{Non-confusion} & good & poor & poor & good & good  \\
        \textbf{Human-like learning} & poor & poor/okay & poor & good* & good  \\ \hline
        \end{tabular}%
    }
    \caption{A rough assessment of the skills exhibited by the different main types of LLL mechanisms (replay, regularization, and dynamic architectures), as well as our new conceptual framework and human learning. Where multiple value are given, the performance is mostly approach-specific. For our framework, ``good*'' means expected to be good, or conceptually designed to be good, while ``good'' means experimentally demonstrated to be good. Future research is required to demonstrate true performance. 
    %With regard to the performance of human learning, in Sec.~\ref{sec:parallels} we discuss how not all people may display these properties all the time.
    }

    \label{tab:skills}
\end{table}
